SyncBleed: A Realistic Threat Model and Mitigation Strategy for Zero-Involvement Pairing and Authentication (ZIPA)

Zero Involvement Pairing and Authentication (ZIPA) is a promising technique for auto-provisioning large networks of Internet-of-Things (IoT) devices. Presently, these networks use password-based authentication, which is difficult to scale to more than a handful of devices. To deal with this challenge, ZIPA enabled devices autonomously extract identical authentication or encryption keys from ambient environmental signals. However, during the key negotiation process, existing ZIPA systems leak information on a public wireless channel which can allow adversaries to learn the key. We demonstrate a passive attack called SyncBleed, which uses leaked information to reconstruct keys generated by ZIPA systems. To mitigate SyncBleed, we present TREVOR, an improved key generation technique that produces nearly identical bit sequences from environmental signals without leaking information. We demonstrate that TREVOR can generate keys from a variety of environmental signal types under 4 seconds, consistently achieving a 90-95% bit agreement rate across devices within various environmental sources.

==> review.tex <==


Paper summary
-------------
The paper introduces Trevor, a protocol for secure key generator for passwordless authentication in IoT. State-of-the art solutions enable devices in the same household to generate bits by gathering data from the environment (i.e. sound, electromagnetic radiation, audio, voltage), but require good synchronization. The paper shows how synchronization messages introduce vulnerabilities, and overcomes them by proposing a solution based on principal component analysis.

Strengths
---------
The problem addressed in the paper is relevant and well-motivated. While assuming perfectly synchronized clocks is very common, achieving that requires some hardware, which may be unrealistic when considering low-cost IoT devices. Hence, ZIPA systems include a synchronization phase to overcome this issue. The authors point out how an adversary may use information leaked during the synchronization phase to infer the environmental signals needed to authenticate their own devices as legitimate devices.


The presented solution aims to overcome the need for this synchronization phase, by allowing small, realistic time misalignments. Namely, the authors present a solution based on principal component analysis. Such a technique inherently amplifies differences in measurements of legitimate devices and adversarial devices (that may be placed, for example, outside the household), while tolerating small shifts in the devices’ measurements.


The paper ensures that the proposed solution is feasible for the hardware capabilities of existing IoT devices. It also includes multiple experiments supporting Trevor’s resilience and guarantees.


In addition, the paper is generally well-written, easy to read.

Weaknesses
----------
The main weakness of the paper is that the guarantees of the presented protocol are only proven empirically, and not formally. Both the resilience against various attacks, and the high-bit agreement property, are only supported by experiments.


It would be interesting to see some theory supporting these results. Maybe some requirements on the environment signals such that the guarantees hold, i.e. how much the legitimate environment needs to differ from the outside environment.



Comments for authors
--------------------
There are a few typos in the paper, such as:
* (Abstract): “Our approach avoids transmitting synchronization messages during authentication process” -> the authentication process
* (Intro): “This enhanced usability also improves system’s overall security” -> the systems’
* (Figure 2 caption): “while the adversary’s device fails to authenticate due to being in different environment” -> a different environment
* (Intro): “We present a comprehensive evaluation Trevor” -> on Trevor
* (Secton 2.1): “After receiving authentication request message from device A” -> an authentication request message
* (Section 2.1): “Both devices independently convert the synchronized signal into a bit sequences” -> a bit sequence
* (Section 2.1): “After key reconciliation stage, both devices will hold identical authentication keys” -> after the key reconciliation stage
* (Section 2.2): “which is only slightly different from the contexts of legitimate environment” ->  a legitimate environment 
* (Section 2.2): “passively listening to wireless communications and environmental signal” -> signals
* (Section 2.3): “We use audio as our environmental signal and evaluating the popular Schurmann and Sigg [27] bit quantization algorithm” -> evaluate
* (Section 2.3): “Inside the office, a YouTube video1 is played to mimic a environment with a conversation” -> an environment
* (Section 2.3): “The adversary accomplishes this by estimating the transfer function between the audio signal measured from legitimate device” -> a legitimate device
* (Section 2.3): “We vary the length of synchronization message” -> a synchronization message
* (Figure 4 caption): “to generate bit sequences that with low bit error rate.” -> sequences with low bit error late
* (Figure 4 caption): The plot; The adversary
* (Section 2.4): “the y-axis shows the bit error rate between two legitimate devies” -> devices
* (Section 2.4): “the two popular ZIPA bit quantization algorithm.” -> algorithms
* (Section 2.4): “that that carry the most information” -> that that carry
* (Section 3): “Although devices A and B are within radio transmit range” -> transmission
* (Section 3): “but Trevor also works other kinds of signals” -> works with
* (Section 3): “it is easy to correct simply by inverting” -> easy to correct by
* (Section 3): “For example, one eigenvector may be associated with the largest eigenvalue in covariance matrix” -> the covariance matrix
* (Section 4): “various kinds of environmental signal” -> signals
* (Section 4): “a mobile phone or IoT device that would use ZIPA scheme” -> the ZIPA scheme
* (Section 5): “are bit error rate and pairing success rate” -> the bit error rate and the pairing success rate.
* (Section 5): “We report both bit error rate” -> the bit error rate.
* (Section 5.1): “We attenuated the 60 Hz component because it has a high amplitude and it is common to legitimate and adversary” -> legitimate and adversarial devices
* (Section 5.1): “of whether a devices is” -> a device
* (Section 5.1): “We believe that this is caused from “ -> caused by
* (Section 5.1): “The some of the eigenvectors in the covariance matrices” -> Some of the
* (Figure 12 caption): “bie error rate” -> bit error
* (Section 5.4): “with the difference of” -> a difference of
* (Section 5.5): “how the algorithm performs on realistic application platform” -> on a realistic
* (Section 5.5): “running on Raspberry Pi-based prototype” -> a Raspberry Pi-based prototype
* (Section 5.5): “a pair of authenticators to initiate measure their environmental audio” -> initiate the measuring
* (Section 5.5): “VoltKey [16] exchange” -> exchanges
* (Section 5.5): “Trevor establishes keys far more quickly than VoltKey which show mean run time of around 32 s” -> which shows a mean run time
* (Section 5.5): “Not including acquisition of the audio signal from PyAudio” the acquisition
* (Section 5.5): “not including time taken to acquire audio” -> the time
* (Section 6): “The result is that our methods can produce fewer key bits per second that existing techniques” -> than existing techniques
*


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #944B
===========================================================================

Overall merit
-------------
1. Reject

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
The authors tackle the problem of supporting automated pairing / key generation for IoT devices; in particular, looking to address information leakage during the protocol which could aid the adversary in recovery the generated key. This authors identify the synchronization messages, which exchange partial sample buffers, as the source of this leakage. To defend against this leakage, the authors build TREVOR, a technique that supports building keys with far more loosely synchronized timing between devices sampling the common environmental signals. The authors implement and evaluate TREVOR in a real-world setting.

Strengths
---------
+ Tackles important problem to improve security for IoT key generation
+ New approach for key generation with unsynchronized environmental noise samples

Weaknesses
----------
- Lack of motivation behind time synchronization issue that drives the work (i.e., 100s of ms)
- Lack of clarity of methodology for the attack on ZIPA (Section 2.3)

Comments for authors
--------------------
Thanks for your submission to MobiCom. Given the ever growing set of IoT devices and the need for simple-to-use (and effective) pairing / key generation schemes, it is great to see some more work in this direction.

Honestly, I have to admit that I'm a bit stuck on some of the premise of this work with respect to time synchronization. You mention that: "Without precise time alignment, even up to a few hundred milliseconds of time offset ... may generate mismatched bit sequences." To me, 100s of milliseconds seems like an incredibly large lack of alignment between two devices that are performing this joint protocol based on one device (A) sending another device (B) a request. Can you provide some intuition/citations as to why this is the case? I don't see any measurements presented of these time shifts in practice; there is some analysis of the effects in Figure 5 for shifts from 50ms to 2000ms, but there is no discussion of how we ended up here in the first place.
- When looking at the synchronization issues mentioned in related work, I see that VoltKey [16] mentions "a long latency up to a few milliseconds is common" in Section 3.4 on Time Synchronization.
- Is there a reason why broadcasting a lightweight message over a wireless channels doesn't suffice for such synchronization (avoiding any propagation delays when using audio channels)?

I have some other questions regarding Section 2.3 and the attack on ZIPA, along with various comments/questions, which I've listed below.

**Detailed Comments/Questions**
- I had a few questions regarding the experiments in Section 2.3 to better understand the real threat of synchronization messages:
  * Earlier in Section 2.1, you discuss the use of noise harvesting for ZIPA, but here you have a YouTube video playing to mimic a conversation. Is this a valid setting? How loud was the audio?
  * How close was the YouTube audio source to the victim device that is sending synchronization messages inside the room?
  * How did you collect the training data for the 1024 synchronization messages? Was this generated using the exact same room setup? How would the attacker go about this collection?
- Why is the x-axis in Figure 13 described as "Time (ms)" but "x10^4"? The corresponding text discusses the results of this figure in units of "seconds".
- In Figure 2 you present a house as a legitimate environment, while the evaluation focuses on distances between devices of at most 2m. What is the goal for TREVOR? Does the pairing success rate shown in Table 2 meet that goal? It's great that the adversary was able to achieve a 0% success rate, but I'm curious about the "Medium" case.
- In Section 5.6, you perform tests of randomness through the NIST test suite. What was your methodology here? How many sequences of bits, and how long were the sequences, did you pass through the test suite? What further analysis did you perform in response to an individual test resulting in a failure? How do I interpret the result of TREVOR passing 9/12 tests? Is this good enough?


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #944C
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
The paper deals with device pairing that uses ambient environmental signals to extract secret key bit sequences. It focuses on synchronization required for the bit generation. The authors propose a technique that avoids the need for synchronization messages during the authentication process by constructing keys from unsynchronized environmental signals.

Strengths
---------
- limited implementation

Weaknesses
----------
- niche problem 
- limited novelty 
- unclear security claims

Comments for authors
--------------------
The authors propose a technique that extracts shared keys from unsynchronized sequences. I have several concerns with this approach. First are the security guarantees. It is not clear how much this proposal weakens the key extraction and reduces the key extraction throughput. The same advantage that the technique provides to the pairing parties, it provides to the adversaries as well. The features that are used to extract the shared key might be more or less vulnerable to eavesdropping from different distances and other types of inference. The authors claim that their technique can be used across audio, voltage, em, but provide no analysis if the technique weakens the security e.g., in terms of the distance from which the attacks could be mounted.  

I wasn't convinced that simple synchronization approaches do not work well in this context and that the proposed scheme is needed in the first place. Maybe I am missing something but existing techniques successfully solve the syncrhonization issue via explicit synch messages and using common correlation-based techniques to fine-tune the key extraction.



==> terms.tex <==
Terms:
--Keys: no tokens, identical ones at the end after reconciliation
--Bit sequences: before keys -> it needs to be corrected.
--Device: not authenticator
--authentication: lets not use pairing. 
--misalignment time: self explanatory
--bit quantization: to extract bit sequences. no more bit extraction
we need to define this somewhere (background)


Other things:
--64-bit key?

